DU-Shapley: A Shapley Value Proxy for Efficient Dataset Valuation

We consider the dataset valuation problem, that is, the problem of quantifying the incremental gain, to some relevant pre-defined utility of a machine learning task, of aggregating an individual dataset to others. The Shapley value is a natural tool to perform dataset valuation due to its formal axiomatic justification, which can be combined with Monte Carlo integration to overcome the computational tractability challenges. Such generic approximation methods, however, remain expensive in some cases. In this paper, we exploit the knowledge about the structure of the dataset valuation problem to devise more efficient Shapley value estimators. We propose a novel approximation, referred to as discrete uniform Shapley, which is expressed as an expectation under a discrete uniform distribution with support of reasonable size. We justify the relevancy of the proposed framework via asymptotic and non-asymptotic theoretical guarantees and illustrate its benefits via an extensive set of numerical experiments.

==> paper_icml/macros.tex <==
%% Packages
\usepackage{amsmath, amsthm, amsfonts}
\usepackage{anysize}
\usepackage[utf8]{inputenx}
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{url}
\usepackage[all]{xy}
\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
% \usepackage[left=2cm,right=2cm]{geometry}
% \usepackage[activeacute, english]{babel}
\usepackage{float}
\usepackage{mathtools}
\usepackage{listings}
\usepackage{color}
\usepackage[english]{babel}
\usepackage{amssymb}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
% \usepackage[linesnumbered,lined,boxed,commentsnumbered]{algorithm2e}
% \usepackage{sidecap}
\usepackage{hyperref}
% \usepackage{eurosym}
\usepackage{subcaption}
\usepackage{fancyhdr}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{cleveref}


\definecolor{darkgreen}{RGB}{0,128,0}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{darkblue}{RGB}{0,0,139}
% \renewcommand{\algorithmiccomment}[1]{ \textcolor{darkgreen}{// \texttt{#1}}}%\verb|\textcolor{green}{#1}|}

%% Commands %%
% \newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\normTV}[1]{\left\|#1\right\|_{\mathrm{TV}}}
% \newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\tbtheta}{\tilde{x}}
% \newcommand{\bz}{\B{z}}
\newcommand{\Zrm}{\mathrm{Z}}
% \newcommand{\bx}{\B{x}}
% \newcommand{\by}{\B{y}}
% \newcommand{\dd}{\mathrm{d}}
% \newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rn}{\mathbb{R}^n}
% \newcommand{\grad}{\nabla}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\bthetastar}{\boldsymbol{x^{\star}}}
\newcommand{\subscript}[2]{$#1 _ #2$}
% \newcommand{\oh}{\operatorname{\mathrm{o}}}
% \newcommand{\Oh}{\operatorname{\mathrm{O}}}
% \newcommand{\1}{\mathds{1}}
\newcommand{\X}{\mathscr{X}}
% \newcommand{\R}{\mathbb{R}}
 \newcommand{\PVar}{\operatorname{Var}}
  \newcommand{\var}[1]{\operatorname{Var}\parenthese{#1}}
    \newcommand{\varLigne}[1]{\operatorname{Var}\parentheseLigne{#1}}
    
\newcommand{\Benjamin}[1]{\noindent\textcolor{blue}{$\langle$\textsf{#1}$\rangle$\marginpar{\tiny\bf \textcolor{blue}{B}}}}
\newcommand{\Felipe}[1]{\noindent\textcolor{darkorange}{$\langle$\textsf{#1}$\rangle$\marginpar{\tiny\bf \textcolor{darkorange}{F}}}}
\newcommand{\Maxime}[1]{\noindent\textcolor{red}{$\langle$\textsf{#1}$\rangle$\marginpar{\tiny\bf \textcolor{red}{M}}}}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{remark}{Remark}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{assumption}{Assumption}
% \newtheorem{example}{Example}

% Parenthèses, Crochets et Accolades
% \newcommand{\pr}[1]{\left({#1}\right)}
% \newcommand{\prn}[1]{({#1})}
% \newcommand{\prbig}[1]{\big({#1}\big)}
% \newcommand{\prBig}[1]{\Big({#1}\Big)}
% \newcommand{\prbigg}[1]{\bigg({#1}\bigg)}
% \newcommand{\prBigg}[1]{\Bigg({#1}\Bigg)}
% \newcommand{\br}[1]{\left[{#1}\right]}
% \newcommand{\brn}[1]{[{#1}]}
% \newcommand{\brbig}[1]{\big[{#1}\big]}
% \newcommand{\brBig}[1]{\Big[{#1}\Big]}
% \newcommand{\brbigg}[1]{\bigg[{#1}\bigg]}
% \newcommand{\brBigg}[1]{\Bigg[{#1}\Bigg]}
% \newcommand{\ac}[1]{\left\{{#1}\right\}}
% \newcommand{\acn}[1]{\{{#1}\}}
% \newcommand{\acbig}[1]{\big\{{#1}\big\}}
% \newcommand{\acBig}[1]{\Big\{{#1}\Big\}}
% \newcommand{\acbigg}[1]{\bigg\{{#1}\bigg\}}
% \newcommand{\acBigg}[1]{\Bigg\{{#1}\Bigg\}}
% \newcommand{\normn}[1]{\|{#1}\|}
% \newcommand{\normbig}[1]{\big\|{#1}\big\|}
% \newcommand{\normBig}[1]{\Big\|{#1}\Big\|}
% \newcommand{\normbigg}[1]{\bigg\|{#1}\bigg\|}

% % Quand on râle sur les fractions :
% \newcommand{\nofrac}[2]{{#1}/{#2}}
% % Quand on râle sur les racines carrées :
% \newcommand{\nosqrt}[1]{{#1}^{\half}}

% % Pour discuter entre nous :
% \newcommand{\vp}[1]{\textcolor{blue}{\small\slshape [VP: #1]}}
% % Pour mettre en évidence les modifications :
% \newcommand{\changed}[1]{\textcolor{red}{#1}}
% % Pour les espaces
% \def\eqsp{\;}

% \renewcommandx{\iint}[2][1=]{\ifthenelse{\equal{#1}{}}{[#2]}{[#1:#2]}}

%%%%%%%%%%%%%%%
%% mathbf
\def\bfn{\mathbf{n}}
\def\bfbeta{\boldsymbol{\beta}}
\def\bfx{\mathbf{x}}
\def\xbf{\mathbf{x}}


%%% mathsf
\def \Yy{\mathbf{Y}}
\def \Kk{\mathbf{Y}}
\def\msi{\mathsf{I}}
% \def\msa{\mathsf{A}}
\def\tmsa{\tilde{\msa}}
\def\msd{\mathsf{D}}
\def\msz{\mathsf{Z}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}}
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{o}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
% \def\msx{\mathsf{X}}
% \def\msy{\mathsf{Y}}

%% mathcal
\def\mca{\mathcal{A}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcb{\mathcal{B}}
%\newcommand{\mcb}[1]{\mathcal{B}(#1)}
\def\mcc{\mathcal{C}}
% \def\mcy{\mathcal{Y}}
% \def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}
\def\mct{\mathcal{T}}

%% mathbb

\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}


%%%% mathrm

\def\rmb{\mathrm{b}}
\def\mrb{\mathrm{b}}
\def\mrl{\mathrm{L}}
\def\rml{\mathrm{L}}
\def\rmd{\mathrm{d}}
\def\rmZ{\mathrm{Z}}
\def\mrd{\mathrm{d}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrc{\mathrm{C}}
\def\mrcc{\mathrm{c}}
\def\rmc{\mathrm{C}}
\def\rmC{\mathrm{C}}
\def\rmcc{\mathrm{c}}
\def\rma{\mathrm{a}}
\def\mra{\mathrm{a}}
\def\rmF{\mathrm{F}}
\def\rmE{\mathrm{E}}


\newcommand{\cco}{\llbracket}
\newcommand{\ccf}{\rrbracket}
\newcommand{\po}{\left(}
\newcommand{\pf}{\right)}
\newcommand{\co}{\left[}
\newcommand{\cf}{\right]}
\newcommand{\D}{\mathcal D}
\newcommand{\A}{\mathcal A}
% \newcommand{\M}{\mathcal M}
\newcommand{\na}{\nabla}
\newcommand{\loiy}{\mu_{\mathrm{v}}}
\newcommand{\rem}[1]{\textcolor{red}{(#1)}}



\def\MeasFspace{\mathbb{M}}
\def\xstar{x^\star}
\def\Tr{\operatorname{T}}
\def\trace{\operatorname{Tr}}
% \newcommandx{\functionspace}[2][1=+]{\mathbb{F}_{#1}(#2)}
%% argmin, argmax
\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argsort}{\operatorname*{arg\,sort}}
% \newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\estimateur}[1]{\hat{\pi}_n^N(#1)}
\def\RichR{\operatorname{R}}
\def\piR{\hat{\pi}^{\RichR}}
\def\estimatorRR{\piR}
% \newcommandx{\VarDeux}[3][3=]{\operatorname{Var}^{#3}_{#1}\left\{#2 \right\}}
\newcommand{\VarDeuxLigne}[2]{\operatorname{Var}_{#1}\{#2 \}}
\newcommand{\gramm}{\operatorname{Gramm}}
% \newcommand{\2}[1]{\mathbbm{1}_{\{#1\}}}




\newcommand{\LeftEqNo}{\let\veqno\@@leqno}

\newcommand{\lambdast}{\lambda^{s \rightarrow t}}
\newcommand{\etast}{\eta^{s \rightarrow t}}
\newcommand{\mst}{m^{s \rightarrow t}}
\newcommand{\mun}{m^{1 \rightarrow 2}}
\newcommand{\mdeux}{m^{2 \rightarrow 1}}
\newcommand{\lambdaun}{\lambda^{2 \rightarrow 1}}
\newcommand{\etaun}{\eta^{2 \rightarrow 1}}
\newcommand{\lambdadeux}{\lambda^{1 \rightarrow 2}}
\newcommand{\etadeux}{\eta^{1 \rightarrow 2}}
\newcommand{\mnun}{m^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\etanun}{\eta^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\lambdanun}{\lambda^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\xpinun}{x_{\pi(n+1)}}
\newcommand{\xnun}{x_{n+1}}
\newcommand{\mpinun}{m^{\pi(n+1) \rightarrow n+1}}
\newcommand{\etapinun}{\eta^{\pi(n+1) \rightarrow n+1}}
\newcommand{\lambdapinun}{\lambda^{\pi(n+1) \rightarrow n+1}}
\newcommand{\pinun}{\pi(n+1)}
\newcommand{\vois}{\mathcal{N}}
\newcommand{\mpii}{m^{i \rightarrow \pi(n+1)}}
\newcommand{\etapii}{\eta^{i \rightarrow \pi(n+1)}}
\newcommand{\lambdapii}{\lambda^{i \rightarrow \pi(n+1)}}
\newcommand{\alphahat}{\widehat{\alpha}}
\newcommand{\betahat}{\widehat{\beta}}
\newcommand{\tildegamma}{\widetilde{\gamma}}
\newcommand{\tildeP}{\widetilde{P}}

\newcommand{\myeqref}[1]{Eq.~\eqref{#1}}



%%%% Floating Points Notation

\newcommand{\fpround}[1]{\lfloor #1 \rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\ceilLigne}[1]{\lceil #1 \rceil}
\newcommand{\floorLigne}[1]{\lfloor #1 \rfloor}
\newcommand{\inv}[1]{\frac{1}{#1}}


%voc
\newcommand{\pth}{\ensuremath{p^{\text{th}}}}
\newcommand{\qth}{\ensuremath{q^{\text{th}}}}
\newcommand{\nth}{\ensuremath{n^{\text{th}}}}

%order
\newcommand{\ord}{\ensuremath{\operatorname{ord}}}
\newcommand{\rad}{\ensuremath{\operatorname{rad}}}



% Sets
% \newcommand{\N}{\ensuremath{\mathbb{N}}}
% \newcommand{\Q}{\ensuremath{\mathbb{Q}}}
% \newcommand{\C}{\ensuremath{\mathbb{C}}}

%\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\primes}{\ensuremath{\mathcal P}}

\newcommand{\sfi}{\ensuremath{\mathcal{S}\!\mathcal{F}}}
\newcommand{\sfibt}{\ensuremath{\mathcal{S}\!\mathcal{F}'}}

\newcommand{\reghat}{\widehat{R}}

\newcommand{\reghatn}{\widehat{R}_n}

\newcommand{\arm}{\mathcal{A}}

\newcommand{\mX}{\widehat{X}}
\newcommand{\PE}{\mathbb{E}}
\newcommand{\Ft}{\mathcal{F}}

\newcommand{\Sy}{\mathbf{S}}

\newcommand{\Kfrac}{\mathscr{K}}

% Operands
\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
% \newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
% \newcommandx{\VnormEq}[2][1=V]{\left\| #2 \right\|_{#1}}
\newcommand{\normLigne}[1]{\Vert #1 \Vert}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLignebig}[1]{\big(#1 \big)}
\newcommand{\parentheseLigneBig}[1]{\Big(#1 \Big)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }

% \newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}
\newcommand{\psLigne}[2]{\langle#1,#2 \rangle}
\newcommand{\psmu}[2]{\left\langle#1,#2 \right\rangle_{\mu}}
\newcommand{\psmuLigne}[2]{\langle#1,#2 \rangle_{\mu}}

\newcommand{\eqdef}{\overset{\text{\tiny def}} =}
\newcommand{\defeq}{\overset{\text{\tiny def}} =}

% Relations
\newcommand{\divid}{\mid}
\newcommand{\ndivide}{\nmid}

% Proba
% \newcommand{\proba}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\probaCond}[2]{\mathbb{P}\left( \left. #1  \middle\vert #2 \right.\right)}
\newcommand{\probaLigne}[1]{\mathbb{P}( #1 )}
% \newcommandx\probaMarkovTilde[2][2=]
% {\ifthenelse{\equal{#2}{}}{{\widetilde{\mathbb{P}}_{#1}}}{\widetilde{\mathbb{P}}_{#1}\left[ #2\right]}}
\newcommand{\probaMarkov}[2]{\mathbb{P}_{#1}\left( #2\right)}
\newcommand{\expe}[1]{\PE \left[ #1 \right]}
\newcommand{\expeExpo}[2]{\PE^{#1} \left[ #2 \right]}
\newcommand{\expeLigne}[1]{\PE [ #1 ]}
\newcommand{\expeLine}[1]{\PE [ #1 ]}
\newcommand{\expeMarkov}[2]{\PE_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovLigne}[2]{\PE_{#1} [ #2 ]}
\newcommand{\expeMarkovExpo}[3]{\PE_{#1}^{#2} \left[ #3 \right]}
\newcommand{\probaMarkovTildeDeux}[2]{\widetilde{\mathbb{P}}_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovTilde}[2]{\widetilde{\PE}_{#1} \left[ #2 \right]}

% Landau notation (big O)
\newcommand{\bigO}{\ensuremath{\mathcal{O}}}
\newcommand{\softO}{\Tilde{\ensuremath{\mathcal{O}}}}

% Environments

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%fleche limite
\newcommand{\flecheLimite}{\underset{n\to+\infty}{\longrightarrow}}
\newcommand{\flecheLimiteOption}[2]{\underset{#1\to#2}{\longrightarrow}}
\newcommand{\flecheLimiteHaut}{\overset{n\to+\infty}{\longrightarrow}}


%notation infini
\newcommand{\plusinfty}{+\infty}

%notation egale
\newcommand{\egale}[1]{\ensuremath{\underset{#1}{=}}}

%plusieurs ligne indice
%\sum\limits_{\substack{i=0 \\ i \neq i_0}}^{n}{A_

\newcommand{\hilbert}{\mathcal{H}}


\def\ie{\textit{i.e. }}
\def\cadlag{càdlàg}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}

\def\primr{f_r}
\def\primrO{f_{r_0}}

\newcommand{\indi}[1]{\1_{#1}}
% \newcommandx{\weight}[2][2=n]{\omega_{#1,#2}^N}
\newcommand{\loi}{\mathcal{L}}
\newcommand{\boule}[2]{\operatorname{B}(#1,#2)}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\boulefermee}[2]{\overline{B}(#1,#2)}
\newcommand{\diameter}{\operatorname{diam}}
\newcommand{\deta}{d_{\eta}}

\def\TV{\mathrm{TV}}

\newcommand{\alain}[1]{\todo[color=blue!20]{{\bf AD:} #1}}
\newcommand{\maxime}[1]{\todo[color=blue!20]{{\bf MV:} #1}}
\newcommand{\vincent}[1]{\todo[color=blue!20]{{\bf VP:} #1}}
\newcommand{\aymeric}[1]{\todo[color=blue!20]{{\bf AyD:} #1}}
\newcommand{\eric}[1]{\todo[color=red!20]{{\bf EM:} #1}}

\newcommand{\tcr}[1]{\textcolor{red}{#1}}



\def\as{\ensuremath{\text{a.s.}}}
\def\dist{\operatorname{dist}}

% \newcommandx\sequence[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{( #1_{#2})}}{\ensuremath{( #1_{#2})_{ #2 \in #3}}}}

% \newcommandx\sequencet[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{( #1_{#2})}}{\ensuremath{( #1_{#2})_{ #2 \geq #3}}}}
% \newcommandx\sequence[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}
% \newcommandx\sequenceD[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{( #1)_{ #2 \in #3} }}}

% \newcommandx{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}
% \newcommandx\sequenceDouble[4][3=,4=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ (#1_{#3},#2_{#3}) \}}}{\ensuremath{\{  (#1_{#3},#2_{#3}), \eqsp #3 \in #4 \}}}}
% \newcommandx{\sequencenDouble}[3][3=n\in\N]{\ensuremath{\{ (#1_{n},#2_{n}), \eqsp #3 \}}}

\newcommand{\wrt}{w.r.t.}
\newcommand{\Withoutlog}{w.l.o.g.}
\def\iid{\text{i.i.d.}}
\def\ifof{if and only if}
\def\eg{e.g.}

% \newcommand{\note}[1]{{\textbf{\color{red}#1}}}

\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\normLip}[1]{\left\Vert #1 \right\Vert_{\text{Lip}}}
\newcommand{\normLipLoc}[1]{\left\Vert #1 \right\Vert_{\text{LipLoc}}}

\def\Lip{\operatorname{Lip}}
\def\generator{\mathcal{A}}
\def\generatorsp{\generator^{\sphere^d}}
\def\generatorr{\generator^{\rset^d}}

\def\momentNoise{\mathrm{m}}
\def\bfe{\mathbf{e}}

\def\bfv{\mathbf{v}}
\def\ebf{\mathbf{e}}
\def\vbf{\mathbf{v}}

\def\Id{\operatorname{Id}}

\def\tildetheta{\tilde{\theta}}

\def\calC{\mathcal{C}}

% \newcommandx{\CPE}[3][1=]{{\mathbb E}_{#1}\left[#2 \left \vert #3 \right. \right]} %%%% esperance conditionnelle
% \newcommandx{\CPVar}[3][1=]{\mathrm{Var}^{#3}_{#1}\left\{ #2 \right\}}
% \newcommand{\CPP}[3][]
% {\ifthenelse{\equal{#1}{}}{{\mathbb P}\left(\left. #2 \, \right| #3 \right)}{{\mathbb P}_{#1}\left(\left. #2 \, \right | #3 \right)}}

\def\Ascr{\mathscr{A}}
\def\Dscr{\mathscr{D}}
\def\scrD{\mathscr{D}}
\def\scrA{\mathscr{A}}
\def\scrB{\mathscr{B}}
\def\scrC{\mathscr{C}}
\def\scrT{\mathscr{T}}
\def\scrF{\mathscr{F}}

\def\barL{\bar{L}}

\def\YL{\mathbf{Y}}
\def\XEM{X}
\def\steps{\gamma}
\def\measSet{\mathbb{M}}

\newcommand\Ent[2]{\mathrm{Ent}_{#1}\left(#2\right)}
% \newcommandx{\osc}[2][1=]{\mathrm{osc}_{#1}(#2)}

% \def\Ybar{\bar{Y}}
\def\Id{\operatorname{Id}}
\def\IdM{\operatorname{I}_d}
\newcommand\EntDeux[2]{\Ent_{#1}\left[#2 \right]}
\def\Ltwo{\mathrm{L}^2}
\def\Lone{\mathrm{L}^1}
\newcommand\densityPi[1]{\frac{\rmd #1}{\rmd \pi}}
\newcommand\densityPiLigne[1]{\rmd #1 /\rmd \pi}
\newcommand\density[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand\densityLigne[2]{\rmd #1/\rmd #2}

\def\V{V}
\def\VD{V}
\def\Vsp{V^{\sphere^d}_{\b,\beta}}
\def\Vr{V^{\rset^d}_{\b,\c,\beta}}

\def\Prset{P^{\rset^d}}
\def\Psphere{P^{\sphere^d}}

\def\n{\mathrm{n}}
\def\Vpsi{\psi}
\def\Vkappa{\kappa}
\def\Vkappat{\tilde{\kappa}}
\def\Vchi{\chi}
\def\Vchit{\tilde{\chi}}
\def\Vphi{\phi}
\def\Vrho{\rho}
\def\psiV{\Vpsi}
\def\rhoV{\Vrho}
\def\phiV{\Vphi}
\def\fV{f}
\def\Vf{\fV}
\def\kappaVt{\tilde{\Vkappa}}
\def\kappaV{\Vkappa}
\def\chiV{\Vchi}
\def\chiVt{\Vchit}


\def\a{a}
\def\b{b}
\def\c{c}
\def\e{e}
\def\rU{\mathrm{r}}

\def\domain{\mathrm{D}}

\def\martfg{M^{f,g}}
\newcommand\Ddir[1]{D_{#1}}
\newcommand\maxplus[1]{\parenthese{#1}_+}
\def\Refl{\mathrm{R}}
\def\phibf{\pmb{\phi}}
\def\Gammabf{\mathbf{\Gamma}}

\def\transpose{\operatorname{T}}
\def\v{v}
\def\w{w}
\def\y{y}
\def\z{z}
%%%% bar

\def\bU{\bar{U}}
\def\Ub{\bU}
\def\lambdab{\bar{\lambda}}
\def\blambdab{\bar{\lambda}}
\def\bv{\bar{v}}
\def\vb{\bv}
\def\yb{\bar{y}}
%\def\by{\yb}
\def\Xb{\bar{X}}
%\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\taub{\bar{\tau}}

\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bF{\bar{F}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}

\def\pib{\bar{\pi}}
\def\bpi{\pib}

\def\S{S}

%%%% normal

\def\nE{E}
\def\nF{F}


%%%% tilde

\def\tF{\tilde{F}}
\def\tmsk{\tilde{\msk}}
\def\tW{\tilde{W}}
\def\tvarsigma{\tilde{\varsigma}}
\def\tv{\tilde{v}}
\def\vt{\tv}
\def\yt{\tilde{y}}
\def\ty{\yt}
\def\Mt{\tilde{M}}
\def\tM{\Mt}

\def\tx{\tilde{x}}
\def\xt{\tx}
\def\tbfx{\tilde{\bfx}}
\def\txbf{\tbfx}
\def\Xt{\tilde{X}}
\def\Yt{\tilde{Y}}
\def\Gt{\tilde{G}}
\def\Et{\tilde{E}}
\def\Tt{\tilde{T}}
\def\St{\tilde{S}}
\def\taut{\tilde{\tau}}

\def\tX{\tilde{X}}
\def\tY{\tilde{Y}}
\def\tG{\tilde{G}}
\def\tE{\tilde{E}}
\def\tT{\tilde{T}}
\def\tS{\tilde{S}}
\def\ttau{\tilde{\tau}}


\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\Sb{\bar{S}}
\def\taub{\bar{\tau}}
\def\Hb{\bar{H}}
\def\Nb{\bar{N}}


\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}
\def\bS{\bar{S}}
\def\bSigma{\bar{\Sigma}}
\def\bH{\bar{H}}
\def\bN{\bar{N}}

%%%%%%%%

\def\mgU{\mathrm{m}_{\nabla U}}
\def\MintDrift{I}
\def\CU{C_U}
\def\RU{R_1}
\def\RV{R}
\def\Reps{R_{\epsilon}}
\def\Resp{\Reps}
\def\veps{\varepsilon}
\def\sphere{\mss}

\def\nablaUt{\overline{\nabla U}}
\def\measureSphere{\nu^d}

\def\etaU{\eta}
\def\epsilonU{\epsilon}

\def\Jac{\operatorname{Jac}}
\def\jac{\operatorname{Jac}}
\def\sign{\operatorname{sign}}
\def\rate{\lambda_{\mathrm{r}}}
\def\sigmaS{\sigma^2}

\def\rmD{\mathrm{D}}%%rmd déjà pris
\def\mrd{\mathrm{D}}
\def\mrc{\mathrm{C}}

\def\diag{\Delta_{\rset^d}}

\def\lyap{V}
\def\supp{\mathrm{supp}}
\def\tpi{\tilde{\pi}}

\newcommand\coupling[2]{\Gamma(\mu,\nu)}
\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}
\newcommand\adh[1]{\overline{#1}}
\newcommand{\fracm}[2]{\left. #1 \middle / #2 \right.}
\newcommand{\comp}{\mathrm{c}}
\newcommand{\fraca}[2]{(#1/#2)}
% \newcommand{\half}{{\nicefrac{1}{2}}}
% \newcommandx{\wasserstein}[2][1=2]{\ifthenelse{\equal{#1}{}}{W}{W_{#1}}}
% \newcommandx{\wassersteinLigne}[3][1=\distance,3=]{\mathbf{W}_{#1}^{#3}(#2)}
% \newcommandx{\wassersteinD}[1][1=\distance]{\mathbf{W}_{#1}}
% \newcommandx{\wassersteinDLigne}[1][1=\distance]{\mathbf{W}_{#1}}

\def\ACb{\mathrm{AC}_{\mathrm{b}}}
\def\opK{\mathrm{K}}

\def\poty{H}
\def\diam{\mathrm{diam}}
\def\talpha{\tilde{\alpha}}
\def\Leb{\mathrm{Leb}}
\newcommand{\iintD}[2]{\{#1,\ldots,#2\}}
\def\interior{\mathrm{int}}
\def\iff{ if and only if }

\def\vareps{\varepsilon}
\def\varespilon{\varepsilon}
\def\si{\text{ if } }
\def\projd{\operatorname{proj}^{\msd}}
\def\projp{\operatorname{proj}^{\msp}}
\def\projz{\operatorname{proj}_{\msz}}
\def\Phibf{\mathbf{\Phi}}

\def\th{\tilde{h}}
\def\thg{\th_{\gamma}}
\def\hg{h_{\gamma}}
\def\bgamma{\bar{\gamma}}
\def\bdelta{\bar{\delta}}
\def\tZ{\tilde{Z}}
\def\tP{\tilde{P}}
\def\tQ{\tilde{Q}}

\def\varphibf{\boldsymbol{\varphi}}
\def\InftyBound{c_\infty}
\def\bfz{\mathbf{z}}
\def\zbf{\bfz}
\def\tbfz{\tilde{\mathbf{z}}}
\def\tzbf{\tbfz}

\def\bfr{\mathbf{r}}
\def\rbf{\bfr}
\def\bfm{\mathbf{m}}
\def\rbm{\bfm}

\def\Ltt{\mathtt{L}}
\def\mtt{\mathtt{m}}
\def\Btt{\mathtt{B}}
\def\Mtt{\mathtt{M}}
\def\tMtt{\tilde{\mathtt{M}}}
\def\bMtt{\bar{\mathtt{M}}}

\def\tR{\tilde{R}}
\def\a{\mathbf{a}}
\def\bpg{\overline{p}_{\sigma^2\gamma}}
\def\tw{\tilde{w}}
\def\rmT{\mathrm{T}}
\def\trmT{\tilde{\rmT}}

\def\deltaInf{\bdelta}
\def\tmu{\tilde{\mu}}

\def\cbf{\mathbf{c}}
\def\tcbf{\tilde{\cbf}}
\def\tpi{\tilde{\pi}}

\def\lyapD{\mathpzc{V}}
\def\LyapD{\mathpzc{V}}
\def\VlyapD{\mathpzc{V}}

\def\lyapDs{\mathpzc{V}^*}
\def\LyapDs{\mathpzc{V}^*}
\def\VlyapDs{\mathpzc{V}^*}

\def\tauginf{\tau_{\gamma}^{\infty}}

\def\constMoment{c}
\def\Wn{W^{(n)}}
\def\Wnbf{\mathbf{W}^{(n)}}

\def\wiener{\mathbb{W}}
\def\wienersigma{\mathcal{W}}
\def\proccano{\mathrm{W}}
\def\canoproc{\proccano}

\def\Wbf{\mathbf{W}}
\def\mubf{\boldsymbol{\mu}}
\def\Wbfn{\Wbf^{(n)}}

\def\thetabf{\btheta}
\def\bftheta{\btheta}
\def\tthetabf{\tbtheta}
\def\tbftheta{\tbtheta}

\def\Abf{\mathbf{A}}
\def\bfA{\mathbf{A}}
\def\bfB{\mathbf{B}}
\def\Bbf{\mathbf{B}}
\def\bfa{\mathbf{a}}
\def\bfgamma{\boldsymbol{\gamma}}
\def\gammabf{\bfgamma}
\def\bfrho{\boldsymbol{\rho}}
\def\rhobf{\boldsymbol{\rho}}
\def\bfN{\boldsymbol{N}}
\def\bbfA{\bar{\bfA}}
\def\bbfB{\bar{\bfB}}
\def\bfOne{\boldsymbol{1}}

% Define the notations of prop3
\def\Idp{\mathbf{I}_p}
\def\Yb{Y}
% \def\Yc{\tilde{Y}}
\def\Ybr{\mathrm{Y}}
\def\Ycr{\tilde{\mathrm{Y}}}
\def\Zb{Z}
\def\Zc{\tilde{Z}}

% \newcommand{\txts}{\textstyle}
\def\loiGauss{\mathrm{N}}
\def\tPi{\tilde{\Pi}}
\def\tildeU{V}


\newcommand{\vp}[1]{\textcolor{blue}{[VP: {#1}]}}  % PineGreen
\newcommand{\auchoix}[1]{\textcolor{cyan}{[auchoix: {#1}]}}  % MidnightBlue
% Pour mettre en évidence les modifications :
\newcommand{\note}[1]{\textcolor{red}{\newline[note: {#1}]\hrule}}

% ---------------------
%\hypersetup{colorlinks = true, urlcolor = blue, bookmarksopen = true}

% On définit les ensembles (plutôt utile en mathématiques...):
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\msa}{\mathsf{A}}
\newcommand{\msx}{\mathsf{X}}
\newcommand{\msy}{\mathsf{Y}}
\newcommand{\mcy}{\mathcal{Y}}
\newcommand{\mcx}{\mathcal{X}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Rd}{\mathbb{R}^{d}}

% On définit des commandes générales
\newcommand{\dd}{\mathrm{d}}
% \newcommand{\1}{\mathbbm{1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\T}{\intercal}
\newcommand{\argmin}{\operatornamewithlimits{\arg\min}}
\newcommand{\oh}{\operatorname{\mathrm{o}}}
\newcommand{\Oh}{\operatorname{\mathrm{O}}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\cov}{\operatorname{cov}}
% Pour les indices :
\newcommand{\half}{1/2}  % \nicefrac{1}{2}
% Quand on râle sur les fractions :
\newcommand{\nofrac}[2]{{#1}/{#2}}  % ma commande préférée
\newcommand{\nosqrt}[1]{{#1}^{\half}}  % également très pratique
\newcommand{\txts}{\textstyle}  % l'état de l'art en compression de formule
\newcommand{\eqsp}{\,}  % pour contrôler l'espace
\newcommand{\tb}{\textbullet\,}

% Parenthèses, Crochets et Accolades
\newcommand{\pr}[1]{\left({#1}\right)}
\newcommand{\prn}[1]{({\textstyle{#1}})}
\newcommand{\prbig}[1]{\big({#1}\big)}
\newcommand{\prBig}[1]{\Big({#1}\Big)}
\newcommand{\prbigg}[1]{\bigg({#1}\bigg)}
\newcommand{\prBigg}[1]{\Bigg({#1}\Bigg)}
\newcommand{\br}[1]{\left[{#1}\right]}
\newcommand{\bbr}[1]{\left\{{#1}\right\}}
\newcommand{\brn}[1]{[{\textstyle{#1}}]}
\newcommand{\brbig}[1]{\big[{#1}\big]}
\newcommand{\brBig}[1]{\Big[{#1}\Big]}
\newcommand{\brbigg}[1]{\bigg[{#1}\bigg]}
\newcommand{\ac}[1]{\left\{{#1}\right\}}
\newcommand{\acn}[1]{\{{\textstyle{#1}}\}}
\newcommand{\acbig}[1]{\big\{{#1}\big\}}
\newcommand{\acBig}[1]{\Big\{{#1}\Big\}}
\newcommand{\acbigg}[1]{\bigg\{{#1}\bigg\}}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\normn}[1]{\|{\textstyle{#1}}\|}
\newcommand{\ninf}[1]{\norm{#1}_\infty}
\newcommand{\abs}[1]{\left\lvert{#1}\right\rvert}
\newcommand{\absn}[1]{\lvert{#1}\rvert}
\newcommand{\ps}[2]{\left\langle{#1},{#2}\right\rangle}  % produit scalaire
\newcommand{\psn}[2]{\langle\textstyle{#1},{#2}\rangle}  % produit scalaire

% On définit les commandes sur les symbôles
\newcommand{\gauss}{\mathrm{N}}
% \newcommand{\loiGauss}{\gauss}
\newcommand{\wass}{W_{2}}
% \newcommand{\dwn}{\mathcal{C}_{dwn}}
\newcommand{\up}{\mathscr{C}}
\newcommand{\Adwn}{\mathcal{A}_{down}}
\newcommand{\Aup}{\mathcal{A}_{up}}
% \newcommand{\epsdwn}{\varepsilon^{(dwn)}}
% \newcommand{\epsup}{\varepsilon^{(up)}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\U}{U}
\newcommand{\M}{M}
\newcommand{\lip}{\mathtt{L}}
\newcommand{\barM}{\bar{\mathtt{M}}}
\newcommand{\MU}{M}
\newcommand{\mU}{\mathtt{m}}
\newcommand{\grad}{H}  % \textsl{H}
\newcommand{\tgrad}{\tilde{H}}
\newcommand{\tgradD}{F}
\def\dd{\mathrm{d}}

\newcommand{\qslds}{$\texttt{QLSD}^\star$}
\newcommand{\qsld}{{\texttt{QLSD}}}
\newcommand{\qsldpp}{$\texttt{QLSD}^{++}$}
\newcommand{\qlsds}{$\texttt{QLSD}^\star$}
\newcommand{\qlsdsharp}{$\texttt{QLSD}^{\#}$}
\newcommand{\qlsd}{{\texttt{QLSD}}}
\newcommand{\qlsdpp}{$\texttt{QLSD}^{++}$}
\def\Bs{\Btt^{\star}}
\def\tBs{\tilde{\Btt}^{\star}}
\def\sigmas{\sigma_{\star}}
\def\MH{\Mtt}
\def\tMH{\tMtt}
\def\thetas{\theta^{\star}}
\def\bMH{\bar{\MH}}
\def\Pens{\mathcal{P}}
\def\tkappa{\tilde{\kappa}}
\def\Dg{\mathrm{D}_{\gamma}}
\def\DgZ{\mathrm{D}_{0,\gamma}}
\def\wpN{\wp_N}
\def\card{\mathrm{card}}
\def\wpNn{\wp_{N,n}}
\def\Fs{F^{\star}}
\def\Hs{H^{\star}}
\def\balpha{\bar{\alpha}}


\makeatletter
\newcommand{\ostar}{\mathbin{\mathpalette\make@circled\star}}
\newcommand{\pstar}{\mathbin{\mathpalette\make@circled+}}
\newcommand{\make@circled}[2]{%
  \ooalign{$\m@th#1\smallbigcirc{#1}$\cr\hidewidth$\m@th#1#2$\hidewidth\cr}%
}
\newcommand{\smallbigcirc}[1]{%
  \vcenter{\hbox{\scalebox{0.77778}{$\m@th#1\bigcirc$}}}%
}
\makeatother
\def\ttheta{\tilde{\theta}}

